Survey on Disaster Management Datasets for Remote Sensing Based Emergency Applications

Recent natural disasters have highlighted the urgent need for efficient data-driven approaches to disaster management. Machine learning (ML) and deep learning (DL) techniques have shown considerable promise in enhancing the key phases of disaster management including mitigation, preparedness, detection, response, and recovery. A critical enabler of successful ML or DL based applications in remote sensing, however, is the accessibility and quality of annotated datasets. With the growing availability of high-resolution imagery from unmanned aerial vehicles (UAVs) and satellites, computer vision and remote sensing algorithms have become essential tools for rapid detection, situational assessment, and decision-making in disaster scenarios. This survey provides a comprehensive overview of publicly available image-based datasets relevant to ML/DL-based disaster management pipelines. Emphasis is placed on datasets that support computer vision and remote sensing tasks across all phases of disaster events including pre-disaster, during, and post-disaster. The goal of this work is to serve as a centralized reference for researchers and practitioners seeking high-quality datasets for rapid development and deployment of remote sensing-driven disaster response solutions.

==> sections/appendices.tex <==
%---------------definitions---------
% \subsection{Definitions}
\begin{itemize}
\item \textbf{Disaster}: A disaster is a significant and devastating disruption to the functioning of a community where the capacity of that community is insufficient to cope or recover with its own resources. % Disasters can be caused naturally, man-made, and technological hazards, as well as various factors that influence the exposure and vulnerability of a community.\cite{www.ifrc.org}
\vspace{.2cm}

\item \textbf{Natural Disaster}:  A disaster caused by natural factors called as a natural disaster e.g., earthquake, flood, cyclone \cite{alexander2018natural}.
\vspace{.2cm}

\item \textbf{Man-made disaster}:  A disaster caused because of human activities. Examples may include wars, fire accidents, industrial accidents \cite{mohamed2007overview}.
\vspace{.2cm}
 
\item \textbf{Disaster Management}: is a process of effectively preparing for and responding to disasters. It involves strategically organizing resources to lessen the harm that disasters cause. It also involves a systematic approach to managing the responsibilities of \textbf{disaster prevention}, \textbf{preparedness}, \textbf{response}, and \textbf{recovery} as part of disaster management cycle \cite{alexander2015disaster}.
\vspace{.2cm}  

\item \textbf{Disaster response}:  refers to the actions taken directly before, during or in the immediate aftermath of a disaster \cite{alexander2015disaster}. It can include evacuations, search and rescue missions, and emergency medical assistance. The objective is to save lives, ensure health and safety and to meet the subsistence needs of the people affected.
\vspace{.2cm}

\item \textbf{Geographic Information Systems (GIS):} are computer based tools to manage, analyze, edit, output, and visualize geographic data\cite{burrough2015principles}. GIS store, analyze, and visualize data for geographic positions on Earth’s surface. GIS stands for Geographic Information Systems and is a computer-based tool that examines spatial relationships, patterns, and trends in geography.
\vspace{.2cm}

\item \textbf{Remote Sensing}: the process of detecting and monitoring the physical characteristics of an area by measuring its reflected and emitted radiation at a distance (typically from satellite or aircraft) \cite{zhu2018review}.The collected data is then processed and analyzed to generate valuable information about various aspects of the environment.
\vspace{.2cm}


\item \textbf{NAIP}: National Agricultural Imagery Program, acquires aerial imagery during the agricultural growing seasons in the continental United States\cite{davies2010estimating}. It is administered by the USDA's Farm Service Agency through the Aerial Photography Field Office in Salt Lake City.
\vspace{.2cm}

\item \textbf{Geodata}: Geodata is location information stored in a GIS\cite{teixeira2018qualitative}. By viewing data with a geographic component, we see it through a different lens.
\vspace{.2cm} 

\item \textbf{GIS Mapping}: It was used back in 1854 to map a disease outbreak in the City of London. Fundamentally, we still use this type of spatial analysis today but in a more sophisticated way. In a nutshell, data without spatial reference doesn’t provide geographic context\cite{burrough2015principles}. And without geographic context, you can’t fully understand the world that we live in today.
\vspace{.2cm}

\item \textbf{SpatioTemporal Asset Catalog (STAC)}:
The Spatio-temporal Asset Catalog (STAC) specification provides a common structure for describing and cataloging spatiotemporal assets\cite{9553518}. A spatio-temporal asset is any file that represents information about the earth captured in a certain space and time.
\vspace{.2cm}

\item \textbf{UNISDR}: United Nations Office for Disaster Risk Reduction
\vspace{.2cm} 

\item \textbf{NDVI}: Normalized difference vegetation index is used in understanding vegetation density and assessing changes in plant health. NDVI is calculated as a ratio between the red (R) and near infrared (NIR) values in traditional fashion: (NIR - R) / (NIR + R)
\vspace{.2cm} 


\end{itemize}

%data for all dataset studied
% \caption{full dataset detail. Each row represents a dataset. The \~ in split and size columns indicate that they are, to the best of our knowledge. In the resolution column {\dots} indicate that the resolutions of the image vary. Spatio-temporal indicates that the dataset varies in both spatial and also cover temporal variable.} 

% \caption{full dataset detail. Each row represents a dataset.} %
%---------------supplements------------
% \subsection{Supplements}
% A distribution of datasets with respect to the journals they were published in. The chart lists various academic journals, including ArXiv, ACM Transactions on Machine Learning (TOML), Neural Information Processing Systems (NeurIPS), and others.The percentage of datasets published in each journal and colors within a stack represents a different conference where the dataset was presented. For example, under ACM Transactions on Machine Learning (TOML), the orange colored section represents a 7.32\% of datasets used in this study.

%  While Springer, ArXiv, ACM Transactions on Machine Learning (TOML), IEEE Conference on Pattern Recognition (ICPR) cover the biggest portotion of about 56.1\% of the datasets. The remaining is distributed among other publishers including ICCV, Modis, PLOS ONE, ICLR, and MTBS, Archive of the International Society for Photogrammetry and Remote Sensing (ISPRS), Conference on Computer Vision and Pattern Recognition (CVPR)

% \begin{figure}[!h]
% \centering
% \noindent
% \begin{minipage}[c]{.5\textwidth}
% \centering
%     \includegraphics[width=1.0\linewidth]{resources/figures/journals-distribution.png} 
%     \caption{Most of dataset discussed have associated publications. This figure presents a distribution of datasets with respect to the journals they were published to.}
%     \label{fig:journals-distribution} 
%  \end{minipage}
% \end{figure}
 
